Finite sample rates for logistic regression with small noise or few samples

The logistic regression estimator is known to inflate the magnitude of its coefficients if the sample size $n$ is small, the dimension $p$ is (moderately) large or the signal-to-noise ratio $1/\sigma$ is large (probabilities of observing a label are close to 0 or 1). With this in mind, we study the logistic regression estimator with $p\ll n/\log n$, assuming Gaussian covariates and labels generated by the Gaussian link function, with a mild optimization constraint on the estimator's length to ensure existence. We provide finite sample guarantees for its direction, which serves as a classifier, and its Euclidean norm, which is an estimator for the signal-to-noise ratio. We distinguish between two regimes. In the low-noise/small-sample regime ($\sigma\lesssim (p\log n)/n$), we show that the estimator's direction (and consequentially the classification error) achieve the rate $(p\log n)/n$ - up to the log term as if the problem was noiseless. In this case, the norm of the estimator is at least of order $n/(p\log n)$. If instead $(p\log n)/n\lesssim \sigma\lesssim 1$, the estimator's direction achieves the rate $\sqrt{\sigma p\log n/n}$, whereas its norm converges to the true norm at the rate $\sqrt{p\log n/(n\sigma^3)}$. As a corollary, the data are not linearly separable with high probability in this regime. In either regime, logistic regression provides a competitive classifier.

==> post_review/does_not_interpolate.tex <==
\section{Various}
\subsection{Logistic regression may not minimize the 0/1 loss}

We construct two examples, in which logistic regression does not minimize the 0/1 loss.
Example \ref{exa_not_separate} shows that the constrained version may not separate the data, even if it is separable.
Example \ref{exa_not_minimize} shows that the unconstrained version may not minimize the 0/1 loss if the data is not separable.

\begin{exa}\label{exa_not_separate}
Let $M=1$, i.e. $\|\hat{\gamma}\|_2\leq 1$ and $n=p=2$.
For $\lambda>0$, let $(x_1,y_1):=((1,0),1)$ and $(x_2,y_2):=(\lambda(-1,1),1)$.
To arrive at a contradiction, suppose that the logistic regression estimator $\hat{\gamma}$ correctly predicts both labels.
That is, $\hat{\gamma}_1>0$ and $\hat{\gamma}_2>\hat{\gamma}_1$.
Together with $\|\hat{\gamma}\|_2\leq 1$, this gives $|\hat{\gamma}_1|\leq 1/\sqrt{2}$.
The loss of the logistic regression estimator $\hat{\gamma}$ is:
\[
\log(1+\exp(-\hat{\gamma}_1))+\log(1+\exp(\lambda\hat{\gamma}_1-\lambda\hat{\gamma}_2))
\geq \log(1+\exp(-1/\sqrt{2}))+\log(1+\exp(-\lambda))
\]
However, the vector $e_1:=(1,0)$ achieves the loss:
\[
\log(1+\exp(-1))+\log(1+\exp(\lambda))
\]
For small $\lambda>0$, the loss of $e_1$ is smaller than that of $\hat{\gamma}$, which is a contradiction.
\end{exa}

\begin{exa}\label{exa_not_minimize}
Let $M=+\infty$, i.e. we have unconstrained logistic regression, and $n=3$, $p=2$.
For $\lambda>0$, let $(x_1,y_1):=((1,1),1)$, $(x_2,y_2):=((-1,1),1)$ and $(x_3,y_3):=((0,-2\lambda),1)$.
First, we note that the data is not separable (without intercept), and so a minimizer of the 0/1-loss is for example $e_2=(0,1)$, which gets $2$ out of $3$ labels correct.
However, we can check that for $\lambda>1$, logistic regression only predicts the third label correctly.
To see why, note that the first order condition with respect to the first coordinate gives $\hat{\gamma}_1=0$.
With respect to the second coordinate, at $\hat{\beta}_1=0$, the derivative is:
\[
-\frac{2}{1+\exp(-\hat{\beta}_2)}
+\frac{2\lambda}{1+\exp(2\lambda\hat{\beta}_2)}
\]
At $\hat{\beta}_2=0$, this derivative is positive if $\lambda>1$.
Since the loss function is convex, this implies that $\hat{\beta}_2<0$.
So, the logistic regression estimator only predicts $1$ out of $3$ labels correctly.
\end{exa}

These specific examples occur with probability zero and are only constructed for illustrative purposes.
However, similar examples could be constructed that occur with positive probability.

{\color{purple} While $\hat{\gamma}$ is not a minimizer of the 0/1-loss with positive probability, from our results and the results in \cite{hsu2023sample} ({\color{red} if they were applicable to the probit model)}, it would follow that with high probability, $\hat{\gamma}$ is close to an empirical risk minimizer, as they are both close to the ground truth $\beta^*$.}

It is worth pointing out here that for any linearly separable dataset, there exists a large $M$, such that the estimator $\hat{\gamma}$ separates the data.
In particular, as $M\rightarrow\infty$, $\hat{\gamma}$ converges to the hard-margin support vector machine, see \cite{rosset2003margin}.

\subsection{The estimator is almost surely nonzero}

Here, we show that the logistic regression estimator in \eqref{eq_opt} is almost surely nonzero for any finite radius $M$, as well as the unconstrained version with $M=+\infty$.
That is, we can assume $\hat{\tau}:=\|\hat{\gamma}\|_2>0$ almost surely.

\begin{prop}\label{prop_nonzero}
Let $M>0$ or $M=+\infty$.
Suppose that the distribution of $y_ix_i$ is absolutely continuous w.r.t. the Lebesgue measure. 
Almost surely, $0$ is not a solution to \eqref{eq_opt}.
\end{prop}

\begin{proof}
Choose an arbitrary $M>0$. 
We show that if $0$ is a solution to \eqref{eq_opt}, then an event with probability zero occurs.
For any $M>0$, 0 lies in the interior of the Euclidean ball of radius $M>0$.
So, if $0$ solves \eqref{eq_opt}, by convexity it must be a root of the derivative of the objective function.
This implies that $\sum_{i=1}^ny_ix_i=0$, which occurs with probability zero.
\end{proof}
